A Survey of Sound Source Localization with Deep Learning Methods

This article is a survey on deep learning methods for single and multiple sound source localization. We are particularly interested in sound source localization in indoor/domestic environment, where reverberation and diffuse noise are present. We provide an exhaustive topography of the neural-based localization literature in this context, organized according to several aspects: the neural network architecture, the type of input features, the output strategy (classification or regression), the types of data used for model training and evaluation, and the model training strategy. This way, an interested reader can easily comprehend the vast panorama of the deep learning-based sound source localization methods. Tables summarizing the literature survey are provided at the end of the paper for a quick search of methods with a given set of target characteristics.

==> A Survey of SSL with DL methods (arXiv version)/acronyms.tex <==
\begin{table}[h!]
\caption{Table of acronyms.}
\label{tab:acronyms}
    \begin{tabular}{|lr|}
    \hline
        \textbf{ACCDOA}     & activity-coupled Cartesian direction of arrival \\
        \textbf{AE}         & autoencoder \\
        \textbf{ATF}        & acoustic transfer function \\
        \textbf{ASR} & automatic speech recognition \\
        \textbf{BGRU}       & bidirectional gated recurrent unit \\
        \textbf{BIR}        & binaural impulse response \\
        \textbf{BRIR}       & binaural room impulse response \\
        \textbf{CC}         & cross-correlation \\
        \textbf{CNN}        & convolutional neural network \\
        \textbf{CRNN}       & convolutional recurrent neural network \\
        \textbf{CPS}        & cross power spectrum \\
        \textbf{DCASE}      & Detection and Classification \\
            & of Acoustic Scenes and Events \\
        \textbf{DIRHA}      & distant-speech interaction \\
                            & for robust home applications \\
        \textbf{DL}         & deep learning \\
        \textbf{DNN}        & deep neural network \\
        \textbf{DoA}        & direction of arrival \\
        \textbf{DP-RTF}     & direct-path relative transfer function \\
        \textbf{DRR} & direct-to-reverberant ratio \\
        \textbf{EM}         & expectation maximization \\
        \textbf{ESPRIT}     & Estimation of Signal Parameters \\
                            & via Rotational Invariance Techniques \\
        \textbf{EVD}        & eigenvalue decomposition \\
        \textbf{FFNN}       & feed-forward neural network \\
        \textbf{FOA}        & first-order Ambisonics \\
        \textbf{GAN}        & generative adversarial network \\
        \textbf{GCC}        & generalized cross-correlation \\
        \textbf{GLU}        & gated linear unit \\
        \textbf{GMM}        & Gaussian mixture models \\
        \textbf{GMR}        & Gaussian mixture regression \\
        \textbf{GPU}        & graphical processing unit \\
        \textbf{GRU}        & gated recurrent unit \\
        \textbf{HATS}       & head-and-torso simulator \\
        \textbf{HOA}        & higher-order Ambisonics \\
    \hline
    \end{tabular}
    \begin{tabular}{|lr|}
    \hline
        \textbf{HRTF}       & head-related transfer function \\
        \textbf{ICA}        & independent component analysis \\
        \textbf{ILD}        & interaural level difference \\
        \textbf{IPD}        & interaural phase difference \\
        \textbf{ITD}        & interaural time difference \\
        \textbf{ISM}        & image source method \\
        \textbf{LSTM}       & long short-term memory \\
        \textbf{MHSA}        & multihead self-attention \\
        \textbf{MLP}        & multiLayer Perceptron \\
        \textbf{MOT}        & multi-object tracking \\       \textbf{MUSIC}      & MUltiple SIgnal Classification \\
        \textbf{NLP}        & natural language processing \\
        \textbf{NoS}        & number of sources \\
        \textbf{PHAT}       & PHAse Transform \\
        \textbf{RIR}        & room impulse response \\
        \textbf{RNN}        & recurrent neural network \\
        \textbf{RTF}        & relative transfer function \\
        \textbf{SA}         & self-attention \\
        \textbf{SCM} & spatial covariance matrix \\
        \textbf{SED}        & sound event detection \\
        \textbf{SELD}       & sound event localization and detection \\
        \textbf{SH} & spherical harmonics \\
        \textbf{SMIR}       & spherical microphone impulse response \\
       \textbf{SMN}       & sequence matching network \\ 
        \textbf{SP}        & signal processing \\
        \textbf{SPS}        & spatial pseudo-spectrum \\
        \textbf{SRP}        & steered power response \\
        \textbf{SSL}        & sound source localization \\
        \textbf{STFT}       & short-term Fourier transform \\
        \textbf{TCN}        & temporal convolutional network \\
        \textbf{TDoA}       & time difference of arrival \\
        \textbf{TF}         & time-frequency \\
        \textbf{VAD}        & voice activity detection \\
        \textbf{VAE}        & variational autoencoder \\
        \textbf{WDO}        & W-disjoint orthogonality \\
        \hline
    \end{tabular}
\end{table}


==> A Survey of SSL with DL methods (arXiv version)/perspectives.tex <==
%%% CONCLUSION %%%
\section{Conclusions and perspectives}
\label{sec:conclusion}

In this paper, we have presented a comprehensive overview of the literature on SSL techniques based on DL methods from 2011 to 2021. We attempted to categorize the many publications in this domain according to different characteristics of the methods in terms of source (mixture) configuration, neural network architecture, input data type, output strategy, training and test datasets, and learning strategy. 
%As we have seen through this survey, most research is oriented toward finding an appropriate neural architecture encompassing several constraints (NoS, moving sources, high reverberation, real-time implementation, etc.) More recently, part of the scientific effort has been geared towards the adaptation of systems trained on synthetic data to perform better on real-world data.
Tables~II--V summarize our survey: They gather the references of the reviewed DL-based SSL papers with the main  characteristics of the proposed methods (the ones that were used in our taxonomy of the different methods) being reported into different columns. We believe these tables can be very useful for a quick search of methods with a given set of characteristics.



% New: perspectives

To conclude this survey paper, we can comment on some current trends and draw a series of perspectives on the future directions that would be interesting to investigate to improve the performance of SSL systems and gain a better understanding of their behavior. Note that some of these perspectives appeal to general methodological issues in deep learning that are common to many applications, and some others are more specific to SSL. Note also that this list of research directions is not meant to be exhaustive.

\subsection{Adaptation to (limited sets of) real-world data}
\label{ssec:perspectives-data}

In a general manner, we observe a drop in performance when DNNs trained on simulated data are tested on real-world signals. This effect is well-known in the DL research in general, it is a particular case of the poor generalization capability of DNNs in the case of significant train-test data mismatch \citep{lecun2015deep, goodfellow_deep_2016}. We recall that this problem remains particularly crucial in SSL due to the difficulty of developing massive labeled datasets (i.e., with reliable annotations of ground-truth sources location) and the use of simulated training data. This is valid for training datasets generated using the usual ``shoebox'' acoustic simulations. Such geometry is rarely encountered is real-world environments. Moreover, the placement of the simulated microphone array is often unrealistic (e.g., it is floating in the air, whereas a practical recording device is often positioned on a table, leading to strong reflections). 

A first approach to tackle this problem is to consider more sophisticated room acoustics simulators, capable of taking into account more complex room geometries and acoustic phenomena, such as scattering or diffraction, see the related discussion in Section~\ref{subsec:syntheticData}.
However, this presents the limitation of a heavier computation cost, which should be balanced with the amount of data to be generated. Another line of research is to progressively train the network with more and more realistic signals, e.g., first with signals generated with simulated SRIRs, then fine-tuning the network with signals generated with real SRIRs, then further fine-tuning it with recorded data. This is in line with the general methodology of domain adaptation (DA) \citep{kouw2019review} and transfer learning \citep{bengio2012deep,zhuang2020comprehensive} used in many applications of DL, which aims at improving the performance of a network on a particular domain (in our case, real-world data) after it has been trained on another domain (here, simulated data). For SSL, the idea is to ``optimize'' the model to the target acoustic environment and/or sound sources. DA is a promising research field on its own, and it has only recently attracted the attention of the SSL community. To our best knowledge, the adversarial approach of \citet{moing_data-efficient_2021} and the entropy-based adaptation of \citet{takeda_unsupervised_2017} are the only representatives of DA for SSL. %Therein, an adversarial configuration is used to ``steer'' a parametric deep generative model to produce the features that resemble the target, unlabeled, domain data.}

Another line of research would be to inspire from weakly-supervised SSL methods based on \textit{manifold learning} \citep{laufer2020data}. The general principle is that the high-dimensional multichannel observed data live in a low-dimensional acoustic space, controlled by a limited number of latent variables (mainly, room dimensions, source and microphone positions, and reflection coefficients). This low-dimensional space, or manifold, can be identified using a large set of unlabeled data and unsupervised data dimension reduction techniques. Then a limited set of labeled data can be used to identify the relationship between observed data and source positions ``in the manifold,'' and thus estimate the source positions from new observed data (using, e.g., interpolation techniques). This principle was largely developed by \citet{laufer2020data}, who proposed several non-deep manifold identification techniques and corresponding SSL algorithms. The same principle can be applied with a DL approach, in particular with deep latent-variable generative models such as the VAE, in the line of the semi-supervised VAE-SSL model of \citet{bianco_semi-supervised_2020,bianco2021semi} already mentioned in Section~\ref{sssec:VAE} (see also an example of weakly supervised VAE-based source-filter decomposition of speech signals by \citet{sadok2022}). To our knowledge, SSL based on ``deep manifold learning'' is still a largely under-considered and open topic in the literature, yet it offers a promising direction to deal with limited annotated datasets.


%\subsection{Neural networks process analysis}

%Although some efforts were made in this thesis to analyze the networks behavior and the influence of some hyperparameters, there is still room for in-depth analyses, which would certainly be profitable to understand why some models perform better than others, and how further improvements can be achieved. This analysis concern is at the core of recent deep learning research, because of the neural network's black box nature, and we hereby propose a few targeted points to be analyzed regarding our domain. A first perspective is to interpret the extracted features which allows the networks to perform quite well in a multi-speaker context, for example based on filter visualization techniques \cite{chollet_deep_2017,bach_pixel-wise_2015}. Regarding the improvements obtained in Section~\ref{ss:multiLocalizationfeatureExtractionModule}, one can wonder what are the differences between the extracted feature of the baseline and the one of the new module which leads to such a performance gain. Also, the small variations in the results for the different proposed feature extraction modules push us into looking into the networks behavior when another convolutional block is added or less max-pooling is employed. 
% faire le lien avec multi-task ci-dessous? déplacer?
%In the same vein, it could be very instructive to study the contents of the extracted feature in the multi-task networks, since it proved to be suitable not only for localization but also for counting. While it is obvious that these two tasks are bound in a certain way, the networks seem to extract meaningful patterns in the input features which are somehow beneficial for counting and localization altogether, which is not straightforward to do with our human-crafted algorithms.

%Furthermore, it could be quite insightful to understand how the attention mechanism is able to make use of the inter-frame information. While the behaviors of LSTM layers are a bit more instinctive to understand due to their recurrent processing, it is more complicated to figure out how self-attention scores are computed, and why the emphasis is put on certain frames. A thorough investigation regarding the scores and the computed vectors could reveal interesting properties on the most informative frames for speaker localization. 
%We believe that an extensive analysis effort should be pursued to definitely leverage the remarkable capabilities of neural networks. Not only could it allow to notably improve the accuracy of counting and localization systems, but it could more importantly provide us new considerations to progress in the audio research field.


\subsection{Flexibility of the trained models}

As opposed to conventional SP techniques, which can be parameterized to adapt to the changes in the system setup, DL methods for SSL generally assume identical setups for the training and the inference phase. 
Particularly, the number, geometrical arrangement and the directivity of the microphones composing an array, are usually assumed to be fixed. This is a serious disadvantage, since the network needs to be retrained for different microphone arrays, despite the fact that the task (SSL) remains the same.  A partial remedy is to use array-agnostic inputs, such as Ambisonics, e.g., \citep{adavanne_direction_2018,perotin_crnn-based_2019,grumiaux_improved_2021}, CPS eigenvectors, e.g., \citep{takeda_sound_2016} or spatial pseudo-spectra, e.g., \citep{nguyen_robust_2020,wu2021sound}. Another possibility is to adopt array-invariant techniques from end-to-end multichannel speech enhancement, e.g., \cite{luo2020end}.

Moreover, one could apply transfer learning and DA techniques, discussed previously, that could enable the models trained for a particular microphone array to adapt to another. Such techniques could not only be beneficial for the changes in microphone array setups, but also for the changes in the input signal parameters, such as the sampling rate, frame and overlap length, as well as the type of the STFT window function. A radical approach would be to make the method inherently independent to parameterization, by treating the input signal as a point cloud, as recently suggested by \citet{subramani2021point}.

%Quantification of uncertainty (perhaps already there with VAE etc.?) 


\subsection{Multi-task learning}

Multi-task training is a general methodology to improve the performance of a DNN-based system on a given task by training the model to jointly and simultaneously tackle several other tasks \citep{zhang2021survey,ruder2017overview}. It has been observed in practice that this often leads to better performance on the first target task. This principle is most often implemented in the following manner: An early part of the model (e.g., a common feature extraction module composed of several layers or several layer blocks) is common for the different tasks, then the model splits into different branches, each one specialized in one of the different tasks. The common part is assumed to allow the discovery of an efficient signal representation, and the fact that this representation is used for several downstream tasks somehow reinforce the efficiency of the representation extraction. 

This principle can be applied to SSL. In fact, it has already been extensively illustrated in this survey with the SELD Task of the DCASE Challenge \citep{politis_overview_2020} and the many candidates that have been proposed to this challenge (and that we have reported in this survey). The vast majority of the candidate DNNs follow the above architecture, with a common feature extraction module followed by two SED and SSL branches. In 2021, the ACCDOA representation was adopted by many researchers, see Section~\ref{sssec:output-reg-Cartesian}, and allowed for a joint SED and SSL process up to the very last model layer. We believe that combining the SSL task with other tasks (alternately to SED or in addition to it) such as source separation or ASR could lead to further advances. For example jointly proceeding to source counting in addition to SSL in the work of \citet{grumiaux_improved_2021} was shown to improve the SSL performance (note that here source counting is explicit and high-resolution, i.e., it consists in estimating the number of active sources at the short-term frame level, whereas it is most often implicit and generally made on a much larger time scale in the SELD task of the DCASE Challenge). Other examples of multi-task learning for SSL can be found in the works of \citet{wu_sslide_2021, wu2021sound}. Combining SSL with source separation in a DL framework is further discussed below. 

Somewhat different from multi-task approaches, the end-to-end \emph{task-oriented} learning of the entire processing chain (stacked localization, DoA-parameterized beamforming and ASR blocks) of \citet{subramanian2021directional} represents a refreshing idea to address the lack of DoA-annotated data. For instance, by using pre-trained ASR blocks, and by ``freezing'' all but the localization part of the system during training, one could use the abundant labeled speech corpora as a proxy information for the localization task. Such systems could incorporate both neural network modules and processing blocks based on conventional SP, as discussed in the next subsection.


\subsection{Combination of DL and conventional SP techniques}

In this survey paper, we have seen how the DL-based data-driven approach to the SSL problem has somehow replaced the conventional SP approach over the last decade. Yet, conventional methods are able to ``explicitly'' exploit strong prior knowledge on the physical underlying processes via signal and propagation models, whereas the exploitation of the spatial information contained in the mixture signal is done mostly ``implicitly'' by DNNs. Therefore, a major perspective for SSL is to get the best of both worlds, i.e., the combination of DL with conventional multichannel SP techniques. 

This can be inspired by what has been done in, e.g., speech enhancement and speech/audio source separation. In the single-channel configuration, DL-based speech enhancement and separation are mostly based on the masking approach in the TF domain. Binary masks or soft masks (reminiscent of the well-known single-channel Wiener filter) are estimated with DNNs from the noisy signal and applied to it to obtain a cleaned version, see the review by \citet{wang2018supervised}.
For multichannel speech enhancement and separation, a straightforward approach is to input the multichannel signal in the mask estimation network. However, more clever strategies can be elaborated. For example,  \citet{erdogan2016improved}, \citet{heymann2016neural} and \citet{higuchi2017deep} proposed combining the DNN-based single-channel masking with beamforming techniques \citep{van1988beamforming}. In these works, the TF-domain masks estimated by a DNN are used to select speech-dominant against noise-dominant TF points, which are then used to estimate speech and noise spatial covariance matrices, respectively, which are finally used to build beamforming filters. These papers report better ASR scores than with direct TF masking or basic beamforming applied separately. This approach was extended by \citet{perotin2018multichannel} with an additional first stage of beamforming in the HOA domain to improve the mask estimation. A joint end-to-end optimization of the mask estimator, the beamformer, and possibly an ASR acoustic model, was considered in the TF domain by \citet{meng2017deep} and  \citet{heymann2017beamnet}, and in the time domain by \citet{li2016neural}. Closer to source separation than to beamforming, \citet{nugraha2016multichannel} combined a DNN trained to estimate a clean speech spectrogram from a noisy speech spectrogram with the source separation technique based on the spatial covariance matrix (SCM) model and Wiener filtering of \citet{duong2010un}. \citet{leglaive2019semi} proposed an unsupervised multichannel speech enhancement system combining a VAE for modeling the (single-channel) clean speech signal and the SCM model for modeling the spatial characteristics of the multi-channel signal. 

Although we can find many examples of combination of DL-based and SP-based approaches for beamforming and source separation, to our knowledge and as shown by our survey, this principle has been poorly applied to SSL so far. Yet, powerful deep models, and in particular deep generative models such as GANs \citep{goodfellow_generative_2014}, VAEs \citep{Kingma2014}, and dynamical VAEs \citep{girin2021dynamical} are now avaible to model the temporal and/or spectral characteristics of sounds, and can be combined with SP-based models.  
Morevover, as already mentioned earlier in this survey, the connection between audio source separation, diarization, and SSL is strong, reciprocal (each task can help to solve the other ones), and is already exploited in many conventional systems \citep{vincent2018audio, gannot2017consolidated}. Future works may thus consider jointly sound source localization, diarization and separation/enhancement in an hybrid approach combining powerful DL models and conventional SP techniques. General frameworks for the joint optimization of DNN parameters and ``conventional'' parameters are now established and can be exploited \citep{engel2020ddsp, shlezinger2020model}. 


\subsection{Moving sources and deep tracking}

In this survey, we poorly considered the case of moving sound sources and the necessity to rely in this case on tracking algorithms. These algorithms take as input the results of SSL obtained individually on each time frame and connect them through time. This is generally based on the use of a model of the source dynamics. In the multi-source case, dynamical models are often combined with source appearance models (which would model the sound texture or the different speakers' voice in the case of audio signals), resulting in the formation of source tracks with a consistent source ``identity'' for each of these tracks. Tracking algorithms also estimate the tracks ``birth'' and ``death,'' i.e., the time at which the corresponding sources are activated or inactivated. Such multi-object tracking (MOT) algorithms have a long history and their detailed description is beyond the scope of this paper; for a good overview of this domain, see the review papers of \citet{vo_multitarget_2015} and \citet{luo2021multiple}. 
%In the particular case of speech sources, it could be interesting to incorporate speaker spectral signatures into a tracking system for even better performance, which would bring us at the intersection with speaker recognition and diarization.

More recently, deep approaches to the MOT problem have emerged, an evolution mostly driven by the computer vision community \citep{CIAPARRONE202061}. For example, RNNs have been used in place of the traditional Kalman filter to model object dynamics for MOT in videos, e.g., \citep{babaee2018occlusion, sadeghian2017tracking, liang2018lstm, saleh2021probabilistic, xiang2019online}. The current trend is to replace RNNs with Transformer-like models, as discussed at the end of Section~\ref{ssec:models-attention}, e.g., \citep{xu2021transcenter, sun2020transtrack, meinhardt2021trackformer}.
The combination of a deep appearance model (automatic speaker recognition, SED) with a deep dynamical model in a sound source tracking system is a largely open problem and certainly a key ingredient for future developments in robust multi-source acoustic scene analysis in adverse acoustic environments and complex scenarios. Given the problem of annotated data scarsity in SSL, DL-based sound source localization and tracking may inspire from the unsupervised deep approaches to the MOT problem recently proposed by, e.g., \citep{Luiten_2020_WACV, karthik2020simple, he2019tracking, crawford2020exploiting, lin2022unsupervised}.

